Fast FPGA emulation of analog dynamics in digitally-driven systems

In this paper, we propose an architecture for FPGA emulation of mixed-signal systems that achieves high accuracy at a high throughput. We represent the analog output of a block as a superposition of step responses to changes in its analog input, and the output is evaluated only when needed by the digital subsystem. Our architecture is therefore intended for digitally-driven systems; that is, those in which the inputs of analog dynamical blocks change only on digital clock edges. We implemented a high-speed link transceiver design using the proposed architecture on a Xilinx FPGA. This design demonstrates how our approach breaks the link between simulation rate and time resolution that is characteristic of prior approaches. The emulator is flexible, allowing for the real-time adjustment of analog dynamics, clock jitter, and various design parameters. We demonstrate that our architecture achieves 1% accuracy while running 3 orders of magnitude faster than a comparable high-performance CPU simulation.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

==> extra.tex <==
\subsection{Truncating the Summation}

In order to practically compute Equation~\ref{eqn:outputsuminfinite}, it is necessary to reduce the summation to a finite number of terms.  Truncating to the most recent $n$ pulse responses yields:
\begin{equation}
\label{eqn:outputsumfinite}
\hat{y}\left(t\right) = \tilde{x}_1 \cdot F\left(t-\tilde{t}_1\right) +\sum_{j=2}^{n} \tilde{x}_j \cdot \left(F\left(t-\tilde{t}_j\right)-F\left(t-\tilde{t}_{j-1}\right)\right)
\end{equation}
where the truncation error is given by:
\begin{equation}
\label{eqn:outputresid}
e_{N} = \sum_{j=n+1}^{\infty} \tilde{x}_j \cdot \left(F\left(t-\tilde{t}_j\right)-F\left(t-\tilde{t}_{j-1}\right)\right)
\end{equation}

To bound this error, we make two assumptions.  First, we assume that successive values of $\tilde{t}_j$ are separated by an amount between  $\Delta T_{\mathrm{min}}$ and $\Delta T_{\mathrm{max}}$.  Such limits might correspond, for example, to the frequency range of an oscillator.  Hence
\begin{equation}
\label{eqn:timebnds}
\left(t-\tilde{t}_j\right) \in T_j
\end{equation}
where $T_j = \left[\left(j-1\right)\Delta T_{\mathrm{min}},~j\Delta T_{\mathrm{max}}\right]$.

Second, we assume that the input is bounded; that is $\left|\tilde{x}_j\right| \leq R$ for some finite $R$.  Having made these assumptions,
\begin{equation}
\label{eqn:outputresidbounds}
e_N \leq R\left(\sum_{m=1} \left|F\left(\tau_{m}\right)-F\left(\tau_{m-1}\right)\right|\right)
\end{equation}
where $\tau_0=\left(n-1\right)\Delta T_{\mathrm{min}}$ and $\tau_1, \tau_2, \ldots$~correspond to the local extrema of $F\left(\tau\right)$ after $\tau_0$ (illustrated in Figure~\ref{fig:truncbnd}).  If the sequence is finite, the last point corresponds to the steady-state value of the step response.

\subsection{Quantization Errors}

Quantization of the PWL representation and input history both contribute error, giving rise to a tradeoff between accuracy and hardware utilization.  In our emulator architecture, the quantization of both types of signals are optimized for each pulse response to keep the overall resource utilization low.

\subsubsection{PWL Coefficient Quantization}

We define the fixed-point representation of PWL offsets and slopes by the following equations:
\begin{alignat}{2}
\hat{a}_{ij} &= c_{ij} \cdot 2^{-u_j} &\hspace{5mm} c_{ij} &= \text{round}\left(a_{ij} \cdot 2^{u_j}\right) \\
\hat{b}_{ij} &= d_{ij} \cdot 2^{-v_j} &\hspace{5mm} d_{ij} &= \text{round}\left(b_{ij} \cdot 2^{v_j}\right)
\end{alignat}
where $u_j$ and $v_j$ are integers.  (Note that the rounding operation occurs when the PWL representation is generated, not using FPGA hardware.)  The quantization errors in offset and slope are therefore bounded to half of their respective resolutions:
\begin{equation}
\begin{split}
\left|a_{ij}-\hat{a}_{ij}\right| &\leq 2^{-u_j-1}\\
\left|b_{ij}-\hat{b}_{ij}\right| &\leq 2^{-v_j-1}
\end{split}
\end{equation}
Substituting these results into Equation~\ref{eqn:domainrestrictedy} results in the following bounds for output error attributed to the quantization of offset and slope, respectively:
\begin{equation}
\begin{aligned}
e_{A} &\leq R\left(2^{-u_n-1}+\sum_{j=1}^{n-1}2^{-u_j}\right) \\
e_{B} &\leq R\left(2^{-v_n-1}\Delta\tau_{n}+\sum_{j=1}^{n-1}2^{-v_j}\Delta\tau_{j}\right)
\end{aligned}
\end{equation}
where it has been assumed that all of the PWL segments in $\hat{F}_j$ have the same width $\Delta\tau_j$.

\subsubsection{Input Quantization} Now we consider the error due to the quantization of the input history $\left(\tilde{t}_j, \tilde{x}_j\right)$.  As with PWL quantization, assume the $j$th input segment is quantized as 
\begin{equation}
\begin{aligned}
\hat{t}_j &= p_j \cdot 2^{-w_j} \\
\hat{x}_j &= q_j \cdot 2^{-z_j}
\end{aligned}
\end{equation}
where $\hat{t}_j$, $\hat{x}_j$, $p_j$, $q_j$ are all integers.  Since $\hat{t}_j$ and $\hat{x}_j$ are generated in realtime, we use the most conservative estimate of quantization error to leave open the possibility of using truncation rather than rounding in the FPGA implementation.  Hence:
\begin{equation}
\begin{split}
\left|\hat{t}_{j}-\tilde{t}_{j}\right| &\leq 2^{-w_j}\\
\left|\hat{x}_{j}-\tilde{x}_{j}\right| &\leq 2^{-z_j}
\end{split}
\end{equation}
The total errors due to quantization of input time and value, respectively, are therefore:
\begin{equation}
\begin{aligned}
e_{T} &\leq R\left(2^{-w_n}\cdot\underset{i}{\text{max}}\left|b_{in}\right|+\sum_{j=1}^{n-1}2^{-w_j+1}\cdot\underset{i}{\text{max}}\left|b_{ij}\right|\right) \\
e_{X} &\leq 2^{-z_1}\cdot\mathrm{max}\left|F_1\right|+\sum_{j=2}^{n}2^{-z_j}\cdot \mathrm{max}\left(D_{j,j-1},~D_{j-1,j}\right)
\end{aligned}
\end{equation}
where 
\begin{equation}
D_{ij} = \mathrm{max}\left\{F_i\right\}-\mathrm{min}\left\{F_{j}\right\}
\end{equation}

% \subsection{Compressing the Step Response}

% \begin{figure}
% \includegraphics[width=\columnwidth]{rx_steps}
% \caption{Family of step responses representing the analog dynamics of the high-speed link transceiver model.  Each step is the convolution of a channel step response, computed from measured S-parameters, with the impulse response of the RX CTLE in one of 16 different settings.  In our FPGA emulator, the CTLE dynamics setting can be changed in real-time, without reprogramming the FPGA.}
% \label{fig:stepfam}
% \end{figure}

% In order to use the precomputed step response in FPGA emulations, it must be compressed to fit in a finite amount of memory (ideally, the smallest unit of BRAM).  Our emulator architecture employs a piecewise-linear (PWL) compression scheme on account of its low overhead.

% Examining Equation~\ref{eqn:outputsumfinite}, it is apparent that $F\left(t\right)$ must be computed at $n$ unique times: namely, at $t-\tilde{t}_1,~t-\tilde{t}_2,~\ldots~,~t-\tilde{t}_n$.  Still assuming Equation~\ref{eqn:timebnds} holds, the step responses evaluations can be replaced by domain-restricted versions of $F\left(t\right)$:
% \begin{equation}
% \label{eqn:domainrestrictedy}
% \hat{y}\left(t\right) = \tilde{x}_1 \cdot F_1\left(t-\tilde{t}_1\right) +\sum_{j=2}^{n} \tilde{x}_j \cdot \left(F_j\left(t-\tilde{t}_j\right)-F_{j-1}\left(t-\tilde{t}_{j-1}\right)\right)
% \end{equation}
% where $F_j = F_{\mkern 1mu \vrule height 2ex\mkern2mu T_j}$.

% In our emulator architecture, each of these domain-restricted functions is approximated by a piecewise-linear function $\hat{F}_j$.  As illustrated in Figure~\ref{fig:pwldef}, the value of $\hat{F}_j$ at a given time is the sum of an offset term and a linear correction: 
% \begin{equation}
% \label{eqn:pwldef}
% \hat{F}_j\left(t\right) = a_{ij} + b_{ij}\left(t-\tau_{ij}\right)
% \end{equation}
% where $a_{ij}$, $b_{ij}$, and $\tau_{ij}$ are respectively the offset, slope, and start time of the PWL segment containing $t$.

% Many objective functions could be used in determining the optimal PWL representation; we chose to minimize the maximum deviation:
% % LaTeX reference: https://jcnts.wordpress.com/2009/11/11/formatting-optimization-problems-with-latex/
% \begin{equation}
% \text{minimize}~~\underset{t \in T_j}{\text{max}}~\left|\hat{F}_{j}\left(t\right)-F_j\left(t\right)\right|
% \end{equation}
% As will be shown shortly, this approach enables guaranteed bounds to be placed on the emulation error due to the PWL representation.

% If we make the additional stipulation that the segment start times $\tau_{ij}$ are preselected, the optimization problem can be efficiently solved as a linear program.  This is not a very limiting requirement, because a PWL function is most efficiently implemented on an FPGA when the spacings between PWL segments are all equal, and when the total number of segments is equal to a power of two, say $2^m$.  Hence, we can search over $m$ to find the minimum number of segments required for a particular error budget.

% Suppose that we have used this optimization process to determine $\hat{F}_j$ and that the optimal value is $\hat{s}_j$ (i.e., it is the maximum error after optimization).  From Equation~\ref{eqn:domainrestrictedy}, the total error from PWL approximations is bounded as:
% \begin{equation}
% e_P \leq R\left(\hat{s}_n + 2\cdot \sum_{j=1}^{n-1}\hat{s}_j\right)
% \end{equation}

Since the PWL modules use BRAM, which is synchronous, there is a one-cycle delay from the calculation of the times $t-\hat{t}_j$ to the retrieval of the appropriate value of $\hat{F}_j$.  Hence, it is necessary for the emulation time $t$ to lead the input value $x$ by one clock cycle.  Crucially, this introduces a one-cycle delay in any feedback loop from an emulation signal to emulation time.

In our high-speed link model, the only such feedback is through the DCO input, where the input code sets the oscillator period, thereby affecting the flow of emulation time.  The settling time of this feedback loop is relatively long compared to a single emulation cycle, so the impact of this delay on system dynamics is minimal.

Each computation tap makes use of one or two PWL evaluation modules $\hat{F}_j$; as a result of the sharing scheme depicted, only $N$ are needed (not $2N-1$).  The implementation of this module is shown in Figure~\ref{fig:pwlimplementation}, in which it can be seen that the upper bits of the evaluation time $t-\tilde{t}_j$ are used to select a PWL segment from BRAM, and the lower bits represent time with respect to the start of the segment.

Owing to the use of BRAM to store the PWL segments, two important constraints arise in the PWL representation.  First, the number of PWL segments is restricted to powers of two over some range (e.g., $2^9$-$2^{14}$ for Zynq BRAM).  Second, the segment lengths for a given PWL representation $\hat{F}_j$ must be the same.  If this were not the case, additional circuitry would be required to compute the BRAM address from $t-\tilde(t)_j$.

\subsection{Error Budget}

Automation scripts and parameterization enabled us to generate the emulator from an error budget specified by $e_N$, $e_A$, $e_B$, $e_X$, and $e_T$.  The truncation error term, $e_N$, is of particular importance as it strongly affects the number of terms that must be used in the summation.  We explored the emulator rate and resource utilization as a function of $e_N$, assuming a total error budget of 0.1\% and dividing the remaining budget evenly between the other four error terms.  As shown in Figure~\ref{fig:errbudget}, it is beneficial to allocate most of the error budget to $e_N$, with the optimal value being around NN\%. 

Conventionally, analog dynamics are emulated by finite impulse response (FIR) or infinite impulse response (IIR)first creating an approximate rational transfer function, which is then discretized using a fixed time step.  Discretization methods such as zero-order hold (ZOH) and the bilinear transform (Tustin's method) are common.

The first step can be problematic, since the natural representation of some systems, such as communication channels, is as a measured frequency response; fitting a rational transfer function to such data often leads to high-order, numerically unstable systems.

The second step, discretization to a fixed-timestep, introduces a direct tradeoff between the time resolution of the emulation.  For a given emulator clock frequency, increasing the emulator time resolution by a certain factor will reduce the emulation rate by the same factor. 

being emulated contains a slowly varying signal, it may be more efficient to model varying analog signals subject to slow dynamics, it may well be more 

Freely-driven analog inputs (i.e., those that are not digitally-driven)  can be handled only approximately by our system, although such signals are processed accurately if they are slowly varying.

Equation~\ref{eqn:ydef}, which defines the output of an LTI system in terms of the impulse response, can be equivalently written in terms of the step response using integration by parts:
\begin{equation}
\begin{aligned}
y\left(t\right) = \sum_k \left(F\left(\tau\right)\cdot x\left(t-\tau\right)\Big|_{t-t_{k+1}}^{t-t_k} - \int_{t-t_{k+1}}^{t-t_k} F\left(\tau\right) \cdot x'\left(t-\tau\right)\,d\tau \right)
\end{aligned}
\end{equation}
where $x'\left(t\right)$ is the time derivative of the input.  If $x$ is slowly varying, then $x\left(t_k\right)\approx x\left(t_{k+1}\right)$ and $x'\left(t\right) \approx 0$, meaning that the output is approximately given by
\begin{equation}
y\left(t\right) \approx \sum_k x\left(t_k\right)\cdot\left(F\left(t-t_k\right) - F\left(t-t_{k+1}\right)\right)
\end{equation}
which is the 

Certain nonlinear components with memory can also be represented simply, provided that their memory has a digital character.  For example, the state of a comparator with hysteresis can be represented as a single bit that selects one of two thresholds.  As long as the comparator input is not varying so rapidly that multiple state transitions would occur between emulation cycles, its output will be accurate.

For more general cases, it is 

Last, it is possible to extend our approach to general nonlinear time-invariant (NLTI) systems, although this is only practical in cases with very weak nonlinearity.  Using the Volterra series, the output of an NLTI system with input $x$ and output $y$ can be expressed as:
\begin{equation}
y\left(t\right) = h_0 + \sum_{n=1}^\infty \int\!\int \cdots \int h_n \left(\tau_1, \tau_2, \ldots, \tau_n\right) \prod_{j=1}^n x\left(t-\tau_j\right)\,d\tau_j
\end{equation}
where $h_n$ is the $n$th Volterra kernel.  The $h_0$ kernel can be trivially implemented as an offset, while the $h_1$ kernel can be implemented as a superposition of pulse responses as discussed earlier.  Considering the $h_2$ kernel, its output contribution $y_2$ can be simplified by assuming that $x$ is digitally-driven (Equation~\ref{eqn:xdef}), leading to :
\begin{equation}
\begin{aligned}
y_2\left(t\right) &= \sum_{j,k} x_j x_k \int_{t-t_{j+1}}^{t-t_j} \int_{t-t_{k+1}}^{t-t_k} h_2\left(\tau_1, \tau_2\right)\,d\tau_1 d\tau_2 \\
&= \sum_{j,k} x_j x_k \cdot F_2\left(t-t_{j+1}, t-t_j, t-t_{k+1}, t-t_k\right)
\end{aligned}
\end{equation}
The function $F_2$ is effectively a multidimensional pulse response; it could be precomputed and stored in the emulator using multidimensional lookup tables.  A similar approach could be used to implement $h_3$, $h_4$, etc.

If the input to an analog block is slowly varying, it may very well be more efficient to model the block's dynamics using a conventional fixed time step FIR or IIR filter.  Such an approach is not incompatible with our architecture; all that is needed is to define the filter's fixed-period clock in the time manager.

With this setup, the emulator would occasionally allocate cycles to times corresponding to filter clock edges.  Since the filter clock could be slow on account of its slowly varying input, the emulator throughput would not be significantly degraded.

As an example, consider an input represented as a weighted sum of functions $a_j$ whose weights change only at discrete times $t_k$:
\begin{equation}
x\left(t\right) = \sum_{j,k} x_{jk} \cdot a_{j}\left(t\right) \cdot \left(u\left(t-t_{k}\right) - u\left(t-t_{k+1}\right)\right)
\end{equation}
The output of an LTI system driven by this input is given by:
\begin{equation}
\begin{aligned}
y\left(t\right) &= \sum_{j,k} x_{jk} \cdot \int_{t-t_{k+1}}^{t-t_k} f\left(\tau\right) \cdot a_j\left(t-\tau\right)\,d\tau \\
&= \sum_{j,k} x_{jk} \cdot \left(A_j\left(t, t-t_{k}\right) - A_j\left(t, t-t_{k+1}\right)\right)
\end{aligned}
\end{equation}
where the effective step response of the $j$th basis function, $A_j$, is given by:
\begin{equation}
A_j\left(t, t'\right) = \int_0^{t'} f\left(\tau\right)\cdot a_j\left(t-\tau\right)\,d\tau
\end{equation}
In general, the explicit time dependence of 

\begin{equation}
H_{\text{CTLE}}\left(s\right) = G\cdot\frac{1+s/\omega_z}{\left(1+s/\omega_1\right)\cdot\left(1+s/\omega_2\right)}
\end{equation}
where $\omega_1 = 2\pi \cdot 2\,\mathrm{GHz}$ and $\omega_2 =2\pi\cdot 8\,\mathrm{GHz}$.  In our implementation, the value of $G$ can be varied from 0~dB to -15~dB in 1~dB increments.

\subsection {Fixed-Point Representation}

Fixed-point formats are used throughout the emulator to represent time and analog signal values.  Our generator script determines the number of integer and fractional bits required for each signal based on its range, generally targeting a quantization error of less than 0.01\%.  Hence, the bit width of most fixed-point numbers is around $\left\lceil 1+\mathrm{log}_2 10^4 \right \rceil = 15$.  In generating the fixed-point formats, we prevent overflow by interval arithmetic to determine the exact range of all fixed-point operations.

\subsubsection{Critical Path}
% * <bclim@stanford.edu> 2018-04-22T04:28:30.988Z:
% 
% > Critical Path}
% > The critical timing path of our design was 24.4 ns after running place-and-route.  Of this, 8.39 ns (34\%) was due to the summation of 85 weighted pulse responses, 7.02 ns (29\%) was due to DSP multiply delays, and 2.73 ns (11\%) was due to BRAM delay in the step response lookup tables.
% ---> Not sure this would be interesting
% 
% ^.
The critical timing path of our design was 24.4 ns after running place-and-route.  Of this, 8.39 ns (34\%) was due to the summation of 85 weighted pulse responses, 7.02 ns (29\%) was due to DSP multiply delays, and 2.73 ns (11\%) was due to BRAM delay in the step response lookup tables.

\begin{figure}
\includegraphics[width=\columnwidth]{emulator_time_management}
\caption{The \texttt{time\char`_manager} module controls the flow of time in the emulator.  In every emulation cycle, the TX and RX clocks each request a time step corresponding to their next clock edges; the time manager simply picks the minimum step requested.  Each of the three emulated clock phases is a gated version of \texttt{clk}, enabled when the corresponding time request is granted.}
\label{fig:timeman}
\end{figure}

% \begin{figure}
% \includegraphics[width=\columnwidth]{pwl_table_implementation}
% \caption{Implementation of a piecewise-linear lookup table in the FPGA emulator.  The MSBs of \texttt{diff} are used to determine the address of the segment ROM, which stores \texttt{offset} and \texttt{slope} data, and \texttt{diff} is defined so that the minimum value of \texttt{in} maps to the first entry in the segment ROM.  The purpose of \texttt{out\char`_bias} is to allow the \texttt{offset} value to be biased around zero, reducing the bit width of its fixed-point representation.}
% \label{fig:pwlimp}
% \end{figure}
